IEEE 802.11bd & 5G NR V2X: Evolution of Radio Access Technologies for V2X Communications

With rising interest in autonomous vehicles, developing radio access technologies (RATs) that enable reliable and low latency vehicular communications has become of paramount importance. Dedicated Short Range Communications (DSRC) and Cellular V2X (C-V2X) are two present-day technologies that are capable of supporting day-1 vehicular applications. However, these RATs fall short of supporting communication requirements of many advanced vehicular applications, which are believed to be critical in enabling fully autonomous vehicles. Both DSRC and C-V2X are undergoing extensive enhancements in order to support advanced vehicular applications that are characterized by high reliability, low latency and high throughput requirements. These RAT evolutions---IEEE 802.11bd for DSRC and NR V2X for C-V2X---can supplement today's vehicular sensors in enabling autonomous driving. In this paper, we briefly describe the two present-day vehicular RATs. In doing so, we highlight their inability to guarantee quality of service requirements of many advanced vehicular applications. We then look at the two RAT evolutions, i.e., IEEE 802.11bd and NR V2X and outline their objectives, describe their salient features and provide an in-depth description of key mechanisms that enable these features. While both, IEEE 802.11bd and NR V2X, are in their initial stages of development, we shed light on their preliminary performance projections and compare and contrast the two evolutionary RATs with their respective predecessors.

==> coexistence.tex <==
\section{coexistence}
\cite{Mitneuer86:online} talks of splitting the band between 802.11p and 'newer' technologies. \\

ITS-G5 and LTE-V2V/I/P will share the 5.9 GHz band, with time-limited band split  (safe harbour channels), which transits to shared use of the middle channel, which transits to shared use of all channels \cite{PowerPoi19:online}

Others mention 802.11p can be used for local and short range communications, while C-V2X used for long range cases \textit{find sources} \\

LTE-V2X not proven compatible with ITS-G5 \cite{PowerPoi0:online}, issue as Europe already has significant ITS-G5 deployments with government support \cite{CAR2CARC19:online}

Why not ITS-G5 in the ITS band and 5G (LTE-V2X) in 5G bands? \cite{PowerPoi0:online}https://www.overleaf.com/project/5c2fe328e3ffb44a73a324b8

==> coexistence_commag.tex <==
\section{Coexistence Issues in the ITS Bands}
\subsection{Coexistence between DSRC and LTE-V}
Considering the fact that DSRC-capable equipment have been available for a long time and LTE-V was standardized as recently as 2017, it is possible that DSRC-capable vehicles will be introduced on the roads first, at least in a few countries. Detailed 3GPP studies have shown that with standardization and/or regulatory intervention, DSRC and LTE-V (and possibly future ITS technologies) can coexist in adjacent ITS channels~\cite{techreport}.

While DSRC and LTE-V can use different channels, at least for safety-critical messages~\cite{techreport}, 3GPP also envisions a scenario where DSRC and LTE-V might coexist in the same channel. In this context, 3GPP documents discuss the following~\cite{techreport, R1-1611593};

\begin{itemize}
 \item Because DSRC and LTE-V support similar type of applications, they must both operate as primary users of the designated spectrum.
 \item If short-term\footnote{Here, short-term refers to coexistence approaches that enable two or more technologies to share the spectrum on a packet-by-packet basis. Similarly, long-term approaches indicate those that consider a time-granularity much larger than what is required to transmit one packet.} LTE-V--DSRC coexistence is required, solutions such as those used for License Assisted Access -- Wi-Fi coexistence can be adopted. However, specification of such procedures is outside 3GPP scope~\cite{techreport}.
\end{itemize}

Some preliminary approaches to enable long-term$^2$ LTE-V--DSRC coexistence under study in 3GPP are described next.
\subsubsection{Geo-location based approach}
The LTE-V concept of geo-zoning can be extended to achieve coexistence between DSRC and LTE-V. For example, a geo-location database can assign resource pools to VUEs such that only those resources that are free from DSRC transmissions can be used by LTE-V UEs~\cite{R1-1611593}. 

\subsubsection{Channel sensing based approach}
Channel sensing-based mechanisms can follow a detect-and-vacate approach. If LTE-V and DSRC users operate in the same channel, LTE-V UEs must decode 802.11p preambles, while DSRC devices must (ideally) decode LTE-V signals. However, it is noted in~\cite{R1-1611593} that by the time LTE-V UEs are deployed, DSRC systems may already be in operation. Keeping this in mind, sensing-based coexistence solutions in LTE-V must be backward-compatible, i.e. compatible with DSRC users that cannot decode LTE-V signals.

To summarize, 3GPP identifies a need for short-term and long-term coexistence mechanisms between ITS technologies. However, future 3GPP releases are likely to include only long-term strategies. 

\subsection{Coexistence between Wi-Fi and LTE-V}
Regulators in the US and Europe are considering opening up the $5.9$~GHz ITS band for Wi-Fi-like unlicensed operations. Considering that the ITS band exists for providing safety-critical services, Wi-Fi devices will operate on a secondary basis, i.e. Wi-Fi devices can use the ITS band so long as they do not interfere with LTE-V or DSRC transmissions. Reference~\cite{naik2017coexistence} and the references therein discuss several strategies developed for effective DSRC--WiFi coexistence. However, to the best of our knowledge, no such studies exist in the context of LTE-V and Wi-Fi coexistence. 

\begin{figure}[htb]
 \centering
 \includegraphics[scale=0.5]{./figures/commag1.eps}
 \caption{Packet Delivery Ratio at LTE-V receiver}
 \label{fig:sim-results}
\end{figure}

\begin{table}[htb]
\centering
\caption{Simulation parameters}
\label{table:sim-params}
 \begin{tabular}{|p{1.9cm}|p{1.5cm}|p{1.8cm}|p{1.7cm}|}
  \hline
  \textbf{Parameter} & \textbf{Value} & \textbf{Parameter} & \textbf{Value} \\ \hline \hline
  LTE-V scenario & Highway fast & VUE density & 120 /km \\ \hline
  LTE-V HARQ & No & Path loss model & WINNER+ B1 (LOS)\\ \hline  
  LTE-V ch. BW & $10$~MHz & Wi-Fi ch. BW & $20$~MHz \\ \hline
  LTE-V tx power & $23$~dBm & Wi-Fi tx power & $23$~dBm \\ \hline
  LTE-V traffic & 10 pkts/sec & Wi-Fi traffic & saturated \\ \hline
  \# Wi-Fi clients & 10 & Wi-Fi PHY rate & $24$~Mbps\\ \hline
 \end{tabular}
\end{table}


We consider a scenario where there is a complete overlap between the spectrum used by LTE-V and Wi-Fi devices. The simulation parameters are provided in Table~\ref{table:sim-params}. Fig.~\ref{fig:sim-results} shows the packet delivery ratio (PDR) observed at an LTE-V receiver for the \emph{Highway Fast} scenario~\cite{molina2017lte}. Specifically, the plots show LTE-V performance for the following scenarios:
\begin{itemize}
 \item no Wi-Fi transmitters present,
 \item Wi-Fi transmitters present, but no coexistence mechanism used, 
 \item Wi-Fi transmitters with frame aggregation disabled,
 \item Wi-Fi transmitters with Arbitration Inter-frame Spacing (AIFS) increased to $900~\mu$sec, and
 \item Wi-Fi transmitters with sensing sensitivity reduced to $-82$~dBm.
\end{itemize}
The value of AIFS has been set to $900~\mu$sec following findings in~\cite{naik2017coexistence} where AIFS = $900~\mu$sec is shown to provide sufficient protection to DSRC devices. Setting the sensing sensitivity value to $-96$~dBm corresponds to a sensing range of $320$~meters using the WINNER+ B1 path loss model. The parameter $d_{\textrm{WiFi--LTE-V}}$ indicates the distance between the Wi-Fi AP and the LTE-V receiver at which the PDR performance is examined. All other LTE-V parameters are consistent with~\cite{molina2017lte}. 

As seen in Fig.~\ref{fig:sim-results}, disabling frame aggregation is most effective in reducing the impact of Wi-Fi on LTE-V performance. This is because a Wi-Fi transmitter using frame aggregation continues to access the medium for a large amount of time without sensing the medium between transmissions. In the existing literature~\cite{naik2018coexistence, naik2017coexistence}, it has been shown that sufficient protection can be provided to DSRC devices by increasing the AIFS and reducing the sensing sensitivity of Wi-Fi transmitters when DSRC and Wi-Fi coexist in the same spectrum band. However, it can be observed in Fig.~\ref{fig:sim-results} that reducing the sensing threshold or increasing the AIFS alone are not as effective in protecting LTE-V transmissions. This is because DSRC devices use a \emph{polite} access scheme that backs-off when another transmitter occupies the medium. On the other hand, LTE-V devices transmit on their selected resource irrespective of whether there is an ongoing transmission or not.

\begin{figure}[htb]
 \centering
 \includegraphics[scale=0.5]{./figures/commag2.eps}
 \caption{Percentage drop in PDR relative to Wi-Fi-free LTE-V operations for different Wi-Fi coexistence mechanisms.}
 \label{fig:combined}
\end{figure}

The three mechanisms outlined above can also be combined. Fig.~\ref{fig:combined} shows the percentage drop in LTE-V PDR relative to Wi-Fi-free LTE-V operations for different combinations of the three coexistence mechanisms. The parameter $d_{\textrm{WiFi--LTE-V}}=5$~m and the distance between the LTE-V transmitter and receiver is $100$~m. Fig.~\ref{fig:combined} shows that even after combining all three mechanisms, the percentage drop in LTE-V performance in the presence of Wi-Fi can be brought down only to $18\%$. The resulting PDR at the LTE-V receiver is merely $80.2\%$. Thus, even after combining all coexistence mechanisms that have been shown to be effective for DSRC--Wi-Fi coexistence, sufficient protection cannot be provided to LTE-V users. Furthermore, the use of the aforementioned mechanisms in Wi-Fi is likely to significantly impact Wi-Fi system performance, rendering LTE-V occupied channels useless for Wi-Fi operations.

==> comparison.tex <==
\section{Comparison}
\subsection{802.11p and 802.11bd}
\begin{itemize}
    %\item In 802.11p, only 1 type of channel is specified and it can be categorized as an V2V channel. However in the case of 802.11bd, additional models for V2I and V2P are also studied \cite{11-18-0821-00-0ngv}. Some V2P models are studied in \cite{11-18-1216-01-0ngv}. Reference \cite{11-18-0821-00-0ngv} also proposes to use the C2C channels defined in \cite{11-14-0259-00-0reg} for V2V and V2P, while using the 3GPP V2V outdoor model \cite{www3gppo21:online} for V2I model. V2I requires separate model as the infrastructure stations would be mostly fixed and elevated, which makes the close surroundings virtually free of scatterers \cite{5710954}.
    \item 802.11p didn't have any explicit Doppler mitigation scheme, whereas current discussions for 802.11bd proposes Midambles and results show its efficacy in combating Doppler spread.Even though other techniques like Receiver based DFE (Decision Feedback Equalization) exist, it is not feasible due to its complexity \cite{11-19-0016-00-00bd}.
    %\item There is a proposal to include PHY impairments like non linear Power Amplifier, Carrier Frequency Offset, Phase Noise etc. when considering the channel models, as simulation show a significant degradation in performance when such impairments are present for higher MCS \cite{11-19-0017-04-00bd}. \textit{see if 802.11ac has it as mentioned in the referred document}.
    %\item Current channel models in 802.11p uses a Half-Bathtub profile to model the Doppler Shift. \cite{11-19-0017-04-00bd} proposes to use pure Doppler method for 802.11bd as it is based on the worst case scenario and thus the robustness of the standard can be better evaluated.
    \item 802.11p had only 1 spatial streams (SS), and \cite{11-19-0009-00-00bd} proposes multiple SS for 802.11bd.
    %\item The channel models used by 802.11p \cite{11-14-0259-00-0reg} are tapped-delay models, which are non-geometry based models \cite{DBLP:journals/corr/ViriyasitavatBT15}. Even though in \cite{11-18-0821-00-0ngv}, it is proposed to use the same model for 802.11bd, in \cite{11-19-0034-01-00bd} it is suggested that Geometry-based Stochastic Channel Models (GSCMs)be used instead.\textit{ 3gpp uses GSCM for system level simulations for road traffic ?}
    %\item In \cite{11-18-1994-02-0ngv}, it is said that the C2C channels proposed for 802.11bd \cite{11-14-0259-00-0reg} assumes that ``common Doppler across all taps can be perfectly compensated at the receiver". But, CFO (Carrier Frequency Offset) estimation doesn't always cancel out common doppler and this may affect the receiver's operation. The paper then proposes a C2C model with common doppler for 802.11bd, and the simulation results show 0.5-2dB performance degradation when common Doppler is added to a C2C channel and this is attributed to CFO/CPE (Common Phase Error).

\end{itemize}

 \begin{table}[htb]
     \centering
     \caption{Comparison of 802.11p and 802.11bd}
     \label{table:comparison-802.11p-802.11bd}
     \begin{tabular}{|p{2.2cm}|p{2cm}|p{3.3cm}|}
        \hline
        \textbf{Feature}  & \textbf{802.11p} & \textbf{802.11bd} \\ \hline
        Communication types & Broadcast &  \\ \hline
        Modulation schemes &  &  \\ \hline
        Channel coding  & BCC & LDPC \\ \hline
       % Control & Control: \\ \hline
        Waveform & OFDM & OFDM (backward compatibility) \\ \hline
        Re-transmissions & None & Congestion dependent \\ \hline
        PHY channels &  &  \\ \hline
        Control \& data multiplexing &  &  \\ \hline
        Counter against Doppler & None explicitly & Midambles \\ \hline
        Sub-carrier spacing & 156.25 kHz & 312.5 KHz, 156.25 KHz, 78.125 KHz \\ \hline
        %& & mmWave: 60, 120 kHz \\ \hline
        Channel Models & V2V & V2V, V2P and V2I  \\ \hline
        &  &  \\ \hline
        &  &  \\ \hline
     \end{tabular}
 \end{table}





















==> ngv_biplav.tex <==
\section{IEEE $802.11$bd: Evolution of IEEE $802.11$p}
\label{sec:ngv}

\subsection{Objectives}
\label{sec:ngv-objectives}
During the development of the first V2V communication standard---IEEE 802.11p---the focus was to develop a standard that assisted in  (i) vehicular safety, (ii) better traffic management, and (iii) other applications that add value, such as parking and vehicle diagnostics. The requirements to support reliable V2V communications were set as follows~\cite{11-13-0543-01-0wng}:  \begin{itemize}
    \item To support velocities up to 200 kilometers/hour (kmph),
    \item Response times of around 100 msec,
    \item Communication range of up to 1000 meters.
\end{itemize}

The 802.11p standard derived its PHY and MAC layers from 802.11a, which was the first Wi-Fi standard to operate in the 5 GHz bands. Since then, however, 802.11a has given way to its successors -- 802.11n and 802.11ac. Considering that 802.11p was developed nearly two decades ago, there is an obvious and urgent need to enhance 802.11p such that applications like enhanced safety features, high definition map downloads, autonomous driving assistance, vehicle positioning etc., which are more demanding in terms of their communication requirements, can be supported. While doing so, PHY and MAC features that have been matured in 802.11n and 802.11ac can be leveraged. With this objective, the IEEE 802.11 Next Generation V2X (NGV) Study Group (SG) was formed in March 2018. After the initial feasibility study was completed and the use-cases defined, the IEEE 802.11bd Task Group (a.k.a TGbd) was created in January 2019\footnote{In the remainder of this paper, we use the terms 802.11bd and NGV interchangeably.}. TGbd's approved Project Authorization Request (PAR)~\cite{11-18-0861-09-0ngv} lists it's objectives as follows:
\begin{itemize}
    \item Define at least one mode that achieves at least twice the throughput (at the MAC layer) as compared to 802.11p under scenarios where the relative vehicle speeds are up to 500 kmph.
    \item Define at least one mode that achieves a 3 dB lower sensitivity level (i.e. twice the communication range) than that of 802.11p.
    \item Define at least one form of vehicle positioning in conjunction with V2X communications.
\end{itemize}

In attaining the above three objectives, the new standard, i.e. 802.11bd, must support the following~\cite{11-18-0861-09-0ngv}:
\begin{itemize}
    \item Interoperability: 802.11p devices must be able to decode (at least one mode of) transmissions from 802.11bd devices, and vice-versa.  
    \item Coexistence: 802.11p devices must detect 802.11bd transmissions and defer channel access, and vice-versa.
    \item Backward compatibility: 802.11bd must define at least one mode in which 802.11bd devices can interoperate with 802.11p devices.
    \item Fairness: 802.11bd and 802.11p devices, when operating on the same channel, must get equal opportunities to access the channel.
\end{itemize}

Although 802.11bd is expected to develop mechanisms for the sub-6 GHz band as well as the millimeter wave (mmWave) bands, development of features that operate in the sub-6 GHz bands are given a higher priority~\cite{11-19-0030-02-00bd}. 

A set of use-cases along with their use-cases have been analyzed in \cite{11-18-1072-01-0ngv}. Some of them are Basic Safety Messages (BSM), Multi-Channel Operation (MCO), Infrastructure Applications, Vehicular Positioning and Location etc. For applications that require large data rates at close ranges, 1500 byte packets might be adopted with control packets for longer ranges using the CANbus style frame \cite{CAN_Specification} of 8 - 16 bytes \cite{11-18-1255-00-0ngv}. 

\subsection{Mechanisms}
\label{sec:ngv-mechanisms}
As 802.11bd is expected to be based on the PHY layer of 802.11ac \cite{CAR2CARC19:online}, it is worthwhile to see how 802.11ac performs when downclocked by 2 to fit in 10 MHz of BW while keeping other parameters same as default 802.11ac. We'll denote this by 2*downclocked. downclocking refers to the reducing of the sub-carrier spacing keeping the total number of sub-carriers equal to what the original band would have (64 and 128 sub-carriers for 20 MHz and 40 MHz band respectively). In this case, 802.11ac 2*downclocked means that now the 64 sub-carriers will occupy the 10 MHz band, which usually is allotted 20 MHz of BW in default 802.11ac \textit{(need to include why 10MHz better than 20MHz ?)}. Even with LDPC enabled, 802.11ac 2*downclocked doesn't perform as well as 802.11p's Packet Error Rate (PER) for the smaller packet sizes (300 Bytes) and lower data rates (QPSK 1/2) \cite{11-18-0513-02-0wng}. However, when Midambles and Space Time Block Coding (STBC) using 2 Transmit Antennas are introduced for 802.11ac 2*downclocked, the performance shows a significant improvement and exceeds 802.11p's PER performance with 1 KB packet size and Modulation and Coding Scheme (MCS) = 64 QAM 2/3. This provides a sound logical ground to incorporate newer technologies implemented in 802.11 n/ac/ah/ax for 802.11bd, as it has been proposed in~\cite{11-18-0860-03-0ngv, 11-18-0513-02-0wng}. Some of the potential candidates technologies are:
\begin{itemize}
    \item Low Density Parity Check (LDPC) instead of Binary Convolutional Coding (BCC) for Forward Error Correction (FCC).
    \item If multiple antennas at both the receiver and transmitter are allowed, transmit diversity can be exploited with STBC \cite{jafarkhani2005space} and Cyclic Shift Diversity (CSD), while Maximal Ratio Combining (MRC) will improve reliability through receiver diversity \cite{jadhav2013performance}. It is important to note that while CSD is backward compatible, STBC is not \cite{dammann2003comparison}. \item Midambles are similar to preambles in form and function, with the only difference being it is inserted in between symbols. When using midambles, the preamble will be used for initial channel estimation and the midamble will be used for channel tracking to update the equalizer coefficients. Without midamble, the estimation provided by the preamble at the beginning of the packet is used for compensating every symbol in the packet which is not a good idea if the channel is a fast-varying one \cite{khorov2018tutorial}. In LTE, a similar role is performed by Demodulation Reference Signal (DMRS) . Even though the transmission rate reduces due to midamble insertion, it is compensated by using higher MCS because of the higher reliability afforded due to midamble-aided better channel estimation. Reference~\cite{5172551} analyzes the effect of adding midambles and shows the improvement in BER as a function of the midambles insertion rate (ratio of data symbols to midambles) using one of the earlier WAVE channel models~\cite{4498409}
    \item Dual Sub-Carrier Modulation (DCM) is a technology introduced in 802.11ax that improves reliability through frequency diversity. It involves modulating the same information on two different sub-carriers that are separated in frequency. \textit{see doc 0009 page 11 for more}
    \item Orthogonal Frequency Division Multiplexing (OFDM) configurations other than 64 subcarriers in a 10MHz band are being actively explored. Studies on other downclocked versions of 802.11n/ac/ax to fit in 10 MHz of BW has been done to analyze the impact of Inter Carrier Interference (ICI) due to Doppler spread on the design of 802.11bd tone numerology in \cite{11-18-1553-00-0ngv}. Efficiency of OFDM improves when the carrier spacing is reduced, but this efficiency comes at the cost of higher ICI and channel variation across OFDM symbols \cite{stamoulis2002intercarrier}. Though ``channel variation from symbol to symbol can be partially resolved by channel tracking techniques: midamble, traveling pilots and etc, channel variation within symbol causes unresolvable ICI" \cite{11-18-1553-00-0ngv}. Results presented show that in addition to 20MHz 802.11 n/ac 2*downclocked, 40MHz 802.11 n/ac 4*downclocked also provides good ICI tolerance in both AWGN (Additive White Gaussian Noise) and fading channels.
\end{itemize}

In terms of MAC layer modifications, frame compression and congestion control are a few of the areas that need to be improved with-respect to 802.11p \cite{11-18-0513-02-0wng}. References \cite{Yadumurthy:2005:RMB:1080754.1080757},  \cite{su2007clustering} and \cite{wang2008ieee} provides measures for improving the MAC layer performance of 802.11p, and they are likely to be valid for 802.11bd in the likely case where 802.11bd MAC doesn't undergo a major modification from 802.11p. In [1249]

It is very important while designing a new Physical Layer Convergence Procedure (PLCP) Protocol Data Unit (PPDU) structure for 802.11bd is that in addition to ensuring performance improvements over 802.11p, it also remains backward compatible and is fair to both in terms of channel access. Keeping these objectives in mind, \cite{11-19-0082-01-00bd} proposes a PPDU frame structure that includes two different modulations.
    
\begin{figure}[H]
    \begin{center}
    \includegraphics[scale=0.26, trim={1cm 7cm 1cm 3cm},clip]{0082.pdf}
    \caption{Proposed Frame Structure}
    \label{fig:struc}
    \end{center}
\end{figure}

While 802.11bd devices will be able to decode the new modulation symbols independent of the 802.11p data, the 802.11p devices will sense the channel as busy during the same time and thus will not attempt any new transmissions. The MCS of 802.11p and 802.11bd symbols can be varied according to the proportion of 802.11bd devices in the neighborhood. The requirement for such a waveform is that the total PPDU duration is similar to an 802.11p packet with QPSK 1/2 \cite{11-19-0082-01-00bd}. Additionally, this structure is also compatible with the retransmission technique being discussed in Sec.~\ref{sec:ngv-challenges-interoperability} \cite{11-18-1186-00-0ngv}. If required, the  802.11p and the 802.11bd sections in the frame can be separated by a time-gap. The advantage with this packet structure is that benefits are accrued without the need to change the higher layers, a fundamental requirement for smoother transition between 802.11p and 802.11bd.

\subsection{Challenges}
\label{sec:ngv-challenges}
\subsubsection{Interoperability and Backward Compatibility discussions}
\label{sec:ngv-challenges-interoperability}
One important consideration to be kept in mind is that the already deployed V2X devices using 802.11p protocol should not be left out when the newer devices are deployed, else it might affect it's wide-spread deployment \cite{11-19-0045-00-00bd}. The V2V Notice for Proposed Rule Making (NPRM) released in December 2016 \cite{201631054:online} mentions ``.. interoperability with all other V2V communications technologies transmitting Basic Safety Messages (BSMs)" as one of the requirements for a V2V standard. This puts certain limitations on the design of the PHY and MAC layer of 802.11bd, as introduction of technologies like STBC or modifying the waveform \cite{11-18-1186-00-0ngv} would mean the legacy devices won't be able to decode the messages. Some of the proposals submitted in the 802.11bd group meetings in this aspect are : 
\begin{itemize}
    \item Presently 802.11p applications operate in the channels 172 (Collision Avoidance) and 178 (Control Channel). These two channels can be excluded from the 802.11bd PHY or an efficient coexistence mechanism for 802.11p and 802.11bd needs to be developed. 
    \item In \cite{11-18-0933-00-0ngv}, three modes of operation are suggested for PHY layer compatibility : 
    \begin{itemize}
        \item Legacy Mode for channels 172 and 178, where only 802.11p will operate.
        \item Greenfield Mode for the presently unused channels 174, 180 and 182; where only 802.11bd can operate.
        \item Mixed Mode for partially used channel 176. With 802.11p devices operating here, 802.11bd devices should be able to talk to the 802.11p devices and vice versa.
    \end{itemize}
    \item Modifying the packet structure, whereby error protection parity bits are added to an 802.11p packet \cite{11-18-1214-00-0ngv}, Reed Solomon in this case (Figure \ref{fig:parity1}). The fact that 802.11p has a larger Short Inter-Frame Space (SIFS) (32 us) than the standard 5 GHz SIFS (16 us) is utilized, so that the parity bits are ignored by the legacy 802.11p device's DIFS (DCF Inter-frame Space) state machine.
\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.26, trim={0cm 2cm 0cm 3cm},clip]{images/1214_new.pdf}
    \caption{Parity bits follow the 802.11p frame}
    \label{fig:parity1}
\end{figure}
 
    The parity bits can also be sent separately in a specially marked packet \cite{11-18-1535-01-0ngv}, with the minimum allowed interval of SIFS between them. Block size for generation of parity bits can be made to vary with the channel load and vehicle speed. This approach of adding parity bits also improves the reliability of the channel. Regarding the possibility of a parity packet being accepted as data, a non-desirable outcome, a single byte is added to the parity packet which will result in a definite  Frame Check Sequence (FCS) failure \cite{11-18-1927-00-0ngv}. Reference~\cite{11-18-1927-00-0ngv} also proposes Frame Aggregation (802.11p doesn't support frame aggregation) for larger messages to counter large overhead, but that might lead to loss of backward-compatibility \cite{11-18-2048-00-0ngv}.
    \item Another way is to re-transmit the same packet more than once through an adaptive re-transmission control that depends on the congestion level \cite{11-18-1186-00-0ngv}.
    
    \begin{figure} [htb]
    \centering
    \includegraphics[scale=0.25, trim={0cm 6cm 0cm 5cm},clip]{1186.pdf}
    \caption{Frame structure given in \cite{11-19-0082-01-00bd}\\}
    \label{fig:retrans}
    \end{figure}
   
    
    
    \textit{also in 3gpp ?} Such a method provides gain for both the 802.11p and 802.11bd stations. See section \ref{sec:ngv-performance-reliability} for more details in this regard. With no idle time between the re-transmissions, as described in \cite{11-18-1186-00-0ngv}, it is impossible for the legacy devices to decode them \cite{11-18-1308-02-0ngv}. Thus the packets can be sent as bursts with a gap of SIFS separating them, or send each re-transmission as separate packets as per EDCA (Enhanced DCF Channel Access) channel access scheme \cite{11-18-1577-00-0ngv}.  \textit{LTE also does retransmissions: if possible compare.}
    \item Reference \cite{11-19-0009-00-00bd} proposes a frame format (see Fig.\ref{fig:new_frame_format}) in which the legacy preambles (Legacy-Short Training Field (L-STF), Legacy -Long Term Field (L-LTF) and L-SIG (Legacy-Signal) are included along with 802.11bd preambles in the 802.11bd header so that legacy 802.11p devices can detect 802.11bd transmissions. \textit{slide 13 doc 0009 ??} 802.11ac header is designed in a similar fashion, so that 802.11a and other legacy devices could detect it and back-off when required.
    
    \begin{figure} [htb]
    \includegraphics[scale=0.28, trim={2cm 7cm 0cm 5cm},clip]{0009.pdf}
    \caption{Frame format given in \cite{11-19-0009-00-00bd}}
    \label{fig:new_frame_format}
    \end{figure}    

    
\end{itemize}

%\subsubsection{Channel Models}
%\label{sec:ngv-challenges-channel-models}
%In \cite{11-18-0821-00-0ngv}, it is proposed that the C2C channel models adopted for 802.11p \cite{11-14-0259-00-0reg} be used for 802.11bd V2V and V2P models, and the V2I model be based on the 3GPP outdoor to outdoor channel model \cite{www3gppo21:online}. However, the C2C channel models have a maximum differential speed of 252 kmph, whereas the PAR \cite{11-18-0861-09-0ngv} states that closing speeds up-to 500 kmph will be supported by 802.11bd. \cite{5710954} provides a very good and comprehensive survey on vehicular channel modelling.

\subsubsection{Coexistence}
\label{sec:ngv-challenges-coexistence}
As per the definition of coexistence provided earlier, it refers to the harmonious coexistence of different devices following different standards peacefully without affecting each other's performance. A number of vehicles equipped with 802.11p based DSRC are already on the road \cite{filippiieee802}, and it will be a bad idea for the newer standard to not include them and might even hamper the chances it's widespread acceptance. A similar situation was encountered during the introduction of 802.11ac with 802.11b/g/n neighbours and this was countered with measures like better carrier sensing, an 802.11ac preamble that could be decoded by 802.11a/n devices, and improvements to the RTS/CTS (Request-To-Send/Clear-To-Send) scheme \cite{80211acT9:online}. A similar approach can be applied here, such as the one proposed in \cite{11-19-0018-00-00bd-ngv}. It provides a measure for 802.11bd devices to identify themselves as 802.11bd devices when their neighborhood consists of both 802.11p and 802.11bd devices. This is important as when an 802.11bd device detects a legacy device around it, it uses the 802.11p PPDU to transmit so that legacy 802.11p devices understand what is being transmitted by 802.11bd devices. On receiving this frame in 802.11p format, other 802.11bd devices might assume that the sender was a legacy device; when in fact it was sent by an 802.11bd device. This would lead to 802.11bd devices communicating with each other using legacy frame structure, when they could have used the newer and better 802.11bd structure. To avoid such a scenario, an 802.11bd device can indicate it's 802.11bd capabilities in the following ways using the legacy broadcast PPDU \cite{11-19-0018-00-00bd-ngv}: 
\begin{itemize}
    \item The simplest way would be to indicate using the MAC header.
    \item Modifying the MAC payload is another way.
    \item PHY header could also be used, but it may lead to compatibility issues with 802.11p devices.
\end{itemize}

Reference \cite{11-19-0083-00-00bd} provides a detailed description on how this indication can be done. A timeout mechanism is used to check if 802.11p neighbor still exists: if the counter gets reset, the 802.11bd device will only transmit in 802.11bd PPDU. \textit{didn't understand slides 7 and 8}. Reference~\cite{11-19-0045-00-00bd} proposes that the higher layer profiles like IEEE 1609, SAE etc. decide the frame format (802.11p or 802.11bd) on a packet-by-packet basis. Additionally, to ensure fairness among the legacy and newer devices, 802.11bd can use the same channel access scheme with similar back-off parameters as 802.11p \cite{11-19-0079-00-00bd}.

\textit{MAC layer paper 1249 also has something on coexistence}

\subsection{Performance Projections}
\label{sec:ngv-performance}


\subsubsection{Improvements in terms of Reliability}
\label{sec:ngv-performance-reliability}
As we have seen in the previous section in ~\ref{sec:ngv-challenges-interoperability}, adding of post-packet data and retransmissions improves the PER performance. The re-transmissions appear as independent transmissions for the 802.11p devices and the gain comes from channel diversity. The newer 802.11bd devices can exploit the fact that the packets are retransmissions and use Log-Likelihood Ratio (LLR) combining or other mechanisms. Depending on the number of transmissions, PER improvements range from 0.5 - 1.7 dB for the 802.11p stations, while for 802.11bd stations it is projected to be 3 - 8 dB  \cite{11-18-1577-00-0ngv}. One way to reduce memory requirements imposed by techniques like LLR, is to define a time-bound beyond which older packets won't be stored \cite{11-18-1577-00-0ngv}. Using Reed-Solomon as the outer code to generate parity bits lead to a PER improvement of 1-3 dB \cite{11-18-1214-00-0ngv}, but latency and complexity to implement it might be an issue \cite{11-18-1680-02-0ngv}. The 802.11p based V2X simulator \cite{11-18-1480-01-0ngv} is used to verify the PER performance benefits of the Reed-Solomon parity bit approach in \cite{11-18-1956-00-0ngv}: the gains are not that significant as reported in \cite{11-18-1577-00-0ngv} and this is attributed to the different Doppler values considered for the two scenarios.


\subsubsection{Improvement in terms of Throughput}
\label{sec:ngv-performance-throughput}
In \cite{11-19-0009-00-00bd}, a few techniques have been outlined through which 802.11bd can achieve higher throughput than 802.11p. They are listed below:
\begin{itemize}
    \item Higher MCS is made feasible by midambles as mentioned in Sec. \ref{sec:ngv-mechanisms}. Simulations performed in \cite{11-19-0016-00-00bd} show considerable throughput improvements over 802.11p using 802.11ac with LDPC and midambles (20 MHz BW), even in high Doppler environments. In the Highway Non Line of Sight (NLOS) scenario, 802.11ac with LDPC and Midambles is shown to have around twice the throughput gain using MCS = 256 QAM, one of the design objectives for 802.11bd as per the PAR. However, 256 QAM doesn't perform well in-terms of PER. The VHT-LTF field is reused as midambles.
    \item Multi Spatial Streams (SS). 802.11ac already supports 8 SS, and this drastically improves channel capacity as each stream carries independent data.  
    \item Wider Bandwidth (BW) channels: The 20MHz channels, 175 and 181, may be used for newer V2X applications. In that case, improvements in the STF/LTF and Control Field sequences, along with  the optimization of the Peak to Average Power Ratio (PAPR) through Phase Rotation \cite{11-19-0009-00-00bd} is needed. In line with this idea,  \cite{11-19-0016-00-00bd} proposes a 20MHz PPDU, where the 10 MHz 802.11p preamble is duplicated for the legacy portion and the 20MHz data can use any of the 20MHz numerology from 802.11ac standard. \textit{figure must}. When using wider BW channels,\cite{11-19-0009-00-00bd} suggests Phase Rotation to improve PAPR.
\end{itemize}

\subsubsection{Improvement in terms of Range}:
\label{sec:ngv-performance-range}
The proposals with regards to range improvement listed in \cite{11-19-0009-00-00bd} are:
\begin{itemize}
    \item Though repeated transmissions lead to reduced throughput and increased memory requirements, it can improve the sensing ability at the receiver.
    \item A special frame format called the Extended Range Single User (ER-SU) PPDU in 802.11ax standard has been designed specifically to increase 802.11ax's range \cite{80211axD17:online}. Similarly a specialized frame format for longer ranges can be implemented for 802.11bd, in which case a frame-type indication method is also needed.
    \item Range improvement can be achieved by making the transmission scheme more robust. With this objective, 802.11ax uses DCM which gives it a PER performance gain of around 2 dB \cite{11-15-1068-01-00ax}, and 802.11ah has defined a new MCS = 10 (BPSK 1/2). Similarly, 802.11bd can use DCM and lower data rates (application-specific) to improve range.
    \item Increasing the transmitter power (within the allowed levels). 
\end{itemize}

%NOTE: I think most of the discussions in this sub-section must be moved to the mechanisms section. What I expect you to talk about in this section is how much performance improvement can be gained by using some of the mechanisms. For example, you can summarize all the performance gains related discussions you have mentioned in the Challenges/Mechanisms section (i.e. numbers like 3 dB improvement and so on). If there are any system level performance studies, you must cite them as well here and talk about the findings of such submissions.

\textcolor{red}{Check section VI-E for what I am expecting in this section.}

\subsection{Additional Comments}
\begin{itemize}
    \item 802.11bd in 60 GHz band : The 60 GHz bands carry a lot of potential for V2X applications as it drastically improves data sharing capabilities for low range applications \cite{11-18-1187-03-0ngv} and thereby provides a strong support for relevant V2X applications\cite{Giannetti1999} \cite{4457895}. 
    Some of the advantages that make mm-Wave bands very attractive for V2X applications are:
    \begin{itemize}
    \item A very large spectrum which can provide high data rates using simple modulation techniques \cite{Microsof41:online}.
    \item Small antenna size, an important factor considering V2X communications.
    \item 60 GHz is the only feasible band where applications requiring high-data rates (GBps) like video streaming in infrastructure-to-vehicle (I2V) scenarios can be supported \cite{7442906}.
    \item \textit{European ITS has 60GHZ provisions ? \cite{citsplat42:online}}\\
\end{itemize}
    Some of the potential V2X applications are downloading of high-resolution 3D maps, sharing sensor data with a nearby vehicle or an RSU, etc. The unicast traffic that contains location-based data (direction for navigating, advertisements) can be offloaded to the 60 GHz band \cite{11-18-1977-05-0ngv}. It can be based on 802.11ad or 802.11ay \cite{11-18-1187-03-0ngv}. Else the incorporation of the 60GHz band into V2V communications would obviously involve the need to develop a different PHY and IEEE 1609 layer \cite{11-18-2048-00-0ngv}. In \cite{11-19-0100-00-00bd}, 802.11ad is used to establish transfer speeds up-to 1 GBps between a car travelling at 60 kmph and an Road Side Unit (RSU) for a few seconds, thus showing the potential of 802.11ad in V2I applications. However, one downside of mm-Wave is that it doesn't support transmission over longer distances, and thus it's utility for purely V2V applications might be limited.
    \item Multi-Channel Operation (MCO): MCO means that an 802.11bd station will simultaneously operate on more than one channel. Presently 802.11p applications use a single channel, however it is justified in saying that multi-channel operation will eventually be needed for newer applications having much higher throughput requirements or for a vehicle to use a different service while still being connected to the safety channel. Reference~\cite{11-18-1928-00-0ngv-ngv} shows how the presence of an interferer in the vicinity affects the Signal to Interference plus Noise Ratio (SINR) of an adjacent channel. Thus there is a need to modify the Adjacent Channel Rejection (ACR) and Spectral Emission Mask (SEM) levels. Reference~\cite{11-18-1186-00-0ngv} proposes the control of the power levels of the adjacent service channels so that the performance of another channel is not affected.  Less interference among adjacent channels would lead to better SINR which also translates to improved transmission range. Reference~\cite{11-19-0048-00-00bd} describes an interference mitigation scheme where the PHY layer compares the real-time Received Signal Strength Indicator (RSSI) from the adjacent channels with pre-determined thresholds. In cases where the RSSI is greater than the threshold, the transmission is delayed and sent when the RSSI falls below the threshold. To ensure the unrestricted operation of the safety channel, \cite{11-18-0933-00-0ngv} recommends:
    \begin{itemize}
        \item Disabling reception when one of the channels is transmitting, or
        \item Fix the timings of service channel transmissions.
    \end{itemize}
    IEEE 1609.4 allows channel switching for vehicles with 1 radio by switching between Control Channel (CCH) and Service Channel (SCH), and synchronization is an mportant factor \cite{Machardy2018}. Support for MCO might also require more than 1 radio, and the number of radios is very likely to be an implementation issue and not hard-coded by the standard \cite{11-18-2072-00-0ngv}. 

    \item Positioning in 802.11bd: The inclusion of positioning services in the PAR \cite{11-18-0861-09-0ngv} means that high precision services could be a part of standard V2X services. Possible use cases include lane assistance, tolling, parking etc. and message frequency of up-to 30 MHz might be needed to support it\cite{11-18-1221-00-0ngv}. While 802.11p could provide relative positioning, absolute positioning could be achieved with the help of the infrastructure stations in the 802.11bd network. More details are available in \cite{11-18-1221-00-0ngv} along with two use-cases and their requirements.

Most of the present developmental efforts for 802.11bd is focused on providing a softer transition from 802.11p as coexistence and inter-operability are one of the important objectives mentioned in the PAR. Thus many of the above-mentioned mechanisms also try to provide some kind of benefit to the already deployed 802.11p STAs. As per [], it is a bad idea to just serve the newer vehicles with 802.11bd. As per , V2X standards based on 802.11 based technologies have a evolution path that can also support older technologies. Studies performed in \cite{11-18-1964-00-0ngv} and \cite{11-19-0045-00-00bd} comparing the older generation technologies,  802.11p and C-V2X, show C-V2X to be superior in terms of performance and therefore a lot is riding on 802.11bd if there is to be any chance for an 802.11 based V2X technology being adopted.

\end{itemize}

 \subsection{Comparison with IEEE 802.11p}
 \label{sec:nrv2x-comparison}
 Table~\ref{table:comparison-802.11p-802.11bd} summarizes the key differences between features/mechanisms of 802.11p and 802.11bd.

 \begin{table}[htb]
     \centering
     \caption{Comparison of 802.11p and 802.11bd}
     \label{table:comparison-802.11p-802.11bd}
     \begin{tabular}{|p{2.2cm}|p{2cm}|p{3.3cm}|}
        \hline
        \textbf{Feature}  & \textbf{802.11p} & \textbf{802.11bd} \\ \hline
        Communication bands & 5.9 GHz & 5.9 GHz \& 60 GHz \\ \hline
        Modulation schemes &  &  \\ \hline
        Channel coding  & BCC & LDPC \\ \hline
       % Control & Control: \\ \hline
        Waveform & OFDM & OFDM ( for backward compatibility) \\ \hline
        Re-transmissions & None & Congestion dependent \\ \hline
        PHY channels &  &  \\ \hline
        Control \& data multiplexing &  &  \\ \hline
        Counter against Doppler & None explicitly & Midambles \\ \hline
        Sub-carrier spacing & 156.25 kHz & 312.5 KHz, 156.25 KHz, 78.125 KHz \\ \hline
        %& & mmWave: 60, 120 kHz \\ \hline
        Channel Models & V2V & V2V, V2P and V2I  \\ \hline
        Supported speeds & 252 kmph & 500 kmph  \\ \hline
        Spatial Streams & 1 & Multiple  \\ \hline
     \end{tabular}
 \end{table}

\begin{comment}
NOTE (Read this from the Latex code section): From my understanding of your section so far, all the mechanisms described under the sub-section "PHY layer" fall into mechanisms that can be used only in the Green-field mode, i.e. in a channel on which only NGV devices operate. This true at least for LDPC codes, MIMO (SFBC), OFDM numerologies OR can be used only for the part of the 802.11bd data in Fig. 2. So I have a few questions and suggestions:

Questions:
- In Fig. 2, I am assuming that after 802.11p data, 802.11p receivers will stop listening to the packet (i.e. will not be able to decode the rest of the packet). Is this correct?

- Will midambles only be used for in 802.11bd part of the data? If not (i.e. if they will be used for 802.11p part as well; though I doubt this) what will be the response of 802.11p devices to the midamble?

- Can 802.11p devices decode higher order MCS? I suspect that should be possible. However, higher order MCS cannot be used when the device speeds are high. That is the reason for not using them in the first place in 802.11p. So that would mean higher MCS will be used with midambles, which takes me back to the previous question.

- From my understanding, among all the mechanisms that you have discussed, there are only two schemes that allow both 802.11p and 802.11bd devices to simultaneously receive a packet. The first is the one shown in Fig. 2 and the second is one shown in Fig. 3. Is this correct?

- What is the benefit of Fig. 5? Using that frame structure, the Tx can only communicate with 802.11bd Rx. Even though 802.11p devices will be able to sense and back-off, they will not be able to decode the packet.

Comments:
- You need to elaborate on DCM. I did not see any discussions on DCM after the first mention. Can DCM be used when coexisting with 802.11p on the same channel?

- The MIMO schemes are only briefly mentioned. Have they not been discussed enough in the documents so far? If so, I think it would be of great interest to the readers.

- I think we need to more clearly understand and then discuss the distinction between coexistence and interoperability/backward compatibility. Do you understand this correctly? If so you can explain to me. Because I am a little confused.

Re-structuring the paper: 
I have modified Sec IV.A. a little bit. Feel free to add any more contents. The structure below is for Sec. IV-B, i.e. Mechanisms, onwards.

I suggest that you discuss the frame structure first. That way for all subsequent discussions where you talk about PHY layer mechanisms, you can say that such mechanisms (where relevant) are applicable only to the 802.11bd portion of the data.

Then, I suggest that you talk about midambles. Here, you can start with talking about why 10 MHz is better suited for vehicular environments (you can cite some references for this point) and then say that simply downclocking doesn't help. And that midambles are required. You need to explain right here what midambles are. You have that somewhere in the challenges section. 

Then depending on how much content you have for each of the PHY mechanisms, such as LDPC, DCM, MIMO and MCS, you can create a separate subsubsection, or you can club multiple ones into a single subsubsection whose title can be "Other PHY layer mechanisms".

I suggest that you put discussions on parity bits and duplication (within the Interoperability section) in the Mechanisms. These are two mechanisms that enable backward compatibility/interoperability. 
The part on channel usage (i.e. three modes of operation for PHY layer compatibilty) can remain in challenges. The coexistence part can also remain in challenges.

\end{comment}



